Materializing Knowledge Bases via Trigger Graphs

The chase is a well-established family of algorithms used to materialize Knowledge Bases (KBs), like Knowledge Graphs (KGs), to tackle important tasks like query answering under dependencies or data cleaning. A general problem of chase algorithms is that they might perform redundant computations. To counter this problem, we introduce the notion of Trigger Graphs (TGs), which guide the execution of the rules avoiding redundant computations. We present the results of an extensive theoretical and empirical study that seeks to answer when and how TGs can be computed and what are the benefits of TGs when applied over real-world KBs. Our results include introducing algorithms that compute (minimal) TGs. We implemented our approach in a new engine, and our experiments show that it can be significantly more efficient than the chase enabling us to materialize KBs with 17B facts in less than 40 min on commodity machines.

==> sections/minimization.tex <==
\section{Minimizing TGs} \label{section:minimization}

In the previous section, we have seen how to compute a full EG for a program $P$ and how to test whether an EG is a TG for $P$. However, the full TG may not be minimal, in the sense that it may comprise nodes which can be deleted from the TG without compromising query answering. Let us return to Example~\ref{example:running} and to the TG $G_1$ from Figure~\ref{figure:trigger-graphs}: we can safely ignore the facts associated with the node $u_6$ from $G_1$ and still preserve the answers to all queries over ${(P_1,B)}$. In this section, we show techniques for minimizing TGs.     

We could minimize a TG by employing the strategy presented in Section~\ref{section:trigger-graph} for testing whether an EG of depth $k$ is a TG for a program $P$. 
That is, among all subgraphs of $\full{P}{k}$, choose the minimal one $\phi$, 
which satisfies ${\phi(B) \models \full{P}{k}(B)}$, for each representative instance $B$ of $\full{P}{k}$.
This technique is sound, however, it is computationally expensive, since it requires considering each subgraph of $\full{P}{k}$.
Furthermore, the resulting graph may still comprise unnecessary-- w.r.t. preserving all queries-- nodes. 
Let us return to the TG $G_1$ from Figure~\ref{figure:trigger-graphs}. The brute force technique will result in the subgraph that comprises all the nodes of $G_1$ (as well as the incident edges of those nodes) except from the nodes $u_6$, $u_8$, $u_9$. The resulting subgraph is suboptimal, since the TG $G_2$ from Figure~\ref{figure:trigger-graphs} comprises fewer nodes and thus reasoning over $G_2$ involves no unnecessary rule executions.
%The resulting subgraph is suboptimal, since the TG $G_2$ from Figure~\ref{figure:trigger-graphs} comprises fewer nodes and using this TG we avoid executing the rule $r_2$ over the facts derived by the rule $r_1$. 
%Recall that as we have seen in Example~\ref{example:running}, all facts derived after executing $r_2$ over the facts derived by the rule $r_1$ can be safely ignored without compromising query answering over ${(P_1,B)}$. 

The minimization process is sound if it preserves the answers to all CQs.  
Consider, for example, a program $P$, a TG $G$ for $P$ of depth $k$, a base instance $B$ and a CQ $Q$ over $P$. Assume that there exists a homomorphism from $Q$ into the facts associated with the nodes ${v_1, \dots, v_j, \dots, v_n}$ from $\nodes{G}$. 
Now, consider a second set of nodes ${v_1, \dots, v'_j, \dots, v_n}$, where the node $v_j$ is replaced by $v'_j$.
Assume a variable $x$ occurring in $Q$. Furthermore, assume that $x$ is mapped to a null $\lnu$ occurring in $v_j(B)$ and that $x$ is a shared variable occurring in multiple atoms from $Q$. Then, in order to answer $Q$, there must exist a homomorphism from $v_j(B)$ into $v'_j(B)$ that preserves $\lnu$. Notice that the labeled null $\lnu$ can occur both in $v_j(B)$ and in $v’_j(B)$ if $v_j(B)$ occurs in some factset $u'(B)$, where $u'$ is an ancestor of $Q$. To recap,  we can compute the same answers to $Q$ over the second set of nodes, if there exists a homomorphism from ${v_j(B)}$ into ${v'_j(B)}$ and this homomorphism preserves all the labeled nulls occurring both in  ${v_j(B)}$ and in some $u'(B)$ with   
$u'$ being an ancestor of $Q$.
We refer to such homomorphisms as preserving homomorphisms:  

\begin{definition}
	Let $G$ be a TG, ${u,v}$ be two nodes in $G$ and $B$ be a base instance.
	A homomorphism from $u(B)$ into $v(B)$ is \emph{preserving}, if it preserves 
	each null occurring both in $u(B)$ and in some $u'(B)$ with $u'$ being an ancestor of $u$.
\end{definition}

For example, consider the instances ${B_1^* = \{\rs(c_1,c_2)\}}$ and ${B_2^* = \{\rs(c_2,c_2)\}}$ from the representative instanceset $\mathcal{H}(P)$.  
For $B_1^*$, the instances $u_1(B_1^*)$, $u_3(B_1^*)$ and $u_5(B_1^*)$ are equal to  
${\{ \Rp(c_1,c_2) \}}$, ${\{ \T(c_1,\lnu) \}}$ and ${\{ \T(c_1,c_1) \}}$, respectively.
For $B_2^*$, the instances $u_1(B_2^*)$, $u_3(B_2^*)$ and $u_5(B_2^*)$ are equal to 
${\{ \Rp(c_1,c_2) \}}$, ${\{ \T(c_2,\lnu) \}}$ and ${\{ \T(c_2,c_2) \}}$, respectively.
Above, $\lnu$ is a labeled null. 
There exists a preserving homomorphism from ${u_3(B_1^*)}$ into ${u_4(B_1^*)}$,
since no labeled null is shared between ${u_3(B_1^*)}$ and ${u_1(B_1^*)}$.
For the same reasons, there exists a preserving homomorphism from ${u_3(B_2^*)}$ into ${u_4(B_2^*)}$.    

The above shows that a node $v$ of a TG can be ``ignored'' for query answering, if for each base instance $B$ of $P$, there exists a node $v'$ and a preserving homomorphism from $v(B)$ into $v'(B)$. Due to the properties of the 
representative instanceset $\repinst{P}{k}$ of $\full{P}{k}$-- recall that $k$ is the depth of $G$--, the above reduces to the following: a node $v$ can be safely ``ignored'' if there exists a node $v'$ and a preserving homomorphism from $v(B)$ into $v'(B)$, for each instance ${B \in \repinst{P}{k}}$. If the above holds, then we say that \emph{$v$ is dominated by $v'$}.  

It may be unsafe to remove the subgraph $G_{\succeq v}$ from the input TG. Consider for example, the TG $G_1$ from Figure~\ref{figure:trigger-graphs}. We can see that there exists a preserving homomophism from $u_3(B)$ into $u_4(B)$ for each ${B \in \mathcal{H}(P)}$. However, we cannot remove the subgraph rooted at 
node $u_3$, since we would also remove the node $u_5$, and hence, we would not preserve the answers to queries involving $\A$-atoms. 
In order to tackle the above problem, we add an edge ${v' \rightarrow_j u}$, for each edge ${v \rightarrow_j u}$ occurring in the original TG. 
This strategy for removing nodes from TGs is described below. 

\begin{definition}\label{definition:minimization}
	The EG $\mathsf{min}(G)$ is obtained from a TG $G$ by exhaustively applying the steps below.  
	For each node ${v \in \nodes{G}}$ that is dominated by another node ${v' \in \nodes{G}}$: (i) remove $v$ from $\nodes{G}$; and (ii)
	add an edge ${v' \rightarrow_j u}$, for each edge ${v \rightarrow_j u}$ from $\edges{G}$.
\end{definition}

The above procedure is sound. 

\begin{restatable}{theorem}{thmminimizeexists}\label{theorem:minimizeexists}
    For each TG $G$ of a program $P$, $\mathsf{min}(G)$ is a TG for $P$.
\end{restatable}

\begin{example}
     We will demonstrate the above minimization process for the TG $G_1$ from Figure~\ref{figure:trigger-graphs}.
     Recall from Example~\ref{example:Trigger-Graph-Computation-Linear} that 
     ${\mathcal{H}(P_1)}$ consists of the instances ${B_1^* = \{\rs(c_1,c_2)\}}$ and ${B_2^* = \{\rs(c_2,c_2)\}}$.
     Since there exists a preserving homomorphism
     from $u_3(B^*)$ into $u_4(B^*)$, for each $B^*$ from ${\mathcal{H}(P_1)}$ 
     we remove $u_3$ from $G_1$ and we copy $u_5$ below $u_4$.
     The output is $G_2$ from Figure~\ref{figure:trigger-graphs}.
\end{example}

\subsection{Minimizing TGs for Datalog programs}  \label{section:minimization:Datalog}

We now turn to the case where $P$ is Datalog. 
%The minimization technique for this case does not require reasoning 
%over the different representative instances and detecting homomorphisms between the instances associated with the nodes of the TG. Instead it reduces to query containment. Hence, it is more efficient.    

The algorithm is based on a simple observation. 
Consider a leaf node $v$ of a TG $G$. Assume that $v$ is associated with the rule ${r(X,Y,Z) \rightarrow R(Y,X)}$. 
For each fact ${r(\sigma(X), \sigma(Y), \sigma(Z))}$ in some base instance $B$,  
where $\sigma$ is a variable substitution, 
the fact ${R(\sigma(Y), \sigma(X))}$ is associated with $v(B)$ when reasoning over the TG. 
Equivalently, for each answer $\sigma$ to ${Q(X,Y) \leftarrow r(X,Y,Z)}$, a
fact ${R(\sigma(Y), \sigma(X))}$ associated with $v(B)$. 

By generalizing the above example, it follows that for each base instance $B$, 
the facts associated with a node $v$ having a head atom $R(\vec{X})$
can be computed by computing all the answers ${\sigma_1,\dots,\sigma_n}$ 
to the rewriting of the query ${Q(\vec{X}) \leftarrow R(\vec{X})}$ over the rules of its ancestors in the TG
and then adding to $v(B)$ each ${\sigma_i(R(\vec{X}))}$. 

In the following, we introduce the notion of a \emph{TG-rewriting}. 
Let $Q$ be a CQ of the form ${Q(\vec{X}) \leftarrow A(\vec{X})}$, where $A(\vec{X})$ is an atom. 
Let $v$ be a node in a TG $G$ associated with a rule $r$ of the form ${\bigwedge \nolimits_{i = i}^n A_i(\vec{Y}_i) \rightarrow A(\vec{Y})}$. 
If the $A_i$-atoms are intensional, we assume that $G$ comprises an edge ${v_i \rightarrow_i v}$, for each $i$. 
Let $\theta$ be the MGU of the set 
${\{\head{r'},A(\vec{X})\}}$, where $r'$ is the rule that results are renaming each variable $Y_i$ in $r$ into a fresh variable $Y'_i$.   

\begin{definition}\label{definition:EP-rewriting}
	The TG-rewriting of $Q$ under ${G_{\preceq v}}$ denoted as ${\rew(Q,G_{\preceq v})}$ is the CQ with head $Q(\theta(\vec{X}))$ and body 
	either \eqref{eq:TG-rewriting:base}, if each $A_i$ is extensional, or \eqref{eq:TG-rewriting:inductive}, if each $A_i$ is intensional.
	\begin{align} 
		\bigwedge \nolimits_{i=1}^n \theta(A_i(\vec{Y}'_i)) \label{eq:TG-rewriting:base} \\
	      \bigwedge \nolimits_{i=1}^n \rew(\theta(Q_i), G_{\preceq v_i}) \label{eq:TG-rewriting:inductive} 
	\end{align}
	In \eqref{eq:TG-rewriting:inductive}, each $Q_i$ is the CQ ${Q_i(\vec{Y}'_i) \leftarrow A_i(\vec{Y}'_i)}$.  
\end{definition}

%Notice that each time we apply Definition~\ref{definition:EP-rewriting}, we rename the variables of the rules associated with the nodes in ${G_{\preceq v}}$ into fresh ones.  

Let $Q$ be the CQ ${Q(\vec{Y}) \leftarrow A(\vec{Y})}$. Recall that $A(\vec{Y})$ is the head of $r$ and that $r$ is the rule associated with $v$. 
We refer to ${\rew(Q,G_{\preceq v})}$ as the \emph{TG-rewriting} of $v$. 

As we show in the appendix, there is a close correspondence between the answers to the TG-rewriting of the node $u$ in $B$ with the data in $u(B)$. 
This correspondence allows us reducing the problem of identifying nodes that can discarded from the TG to the problem of query containment.
The above implies a simple technique for minimizing TGs of Datalog programs.    

%Below, let $Q$ be the CQ ${Q(\vec{Y}) \leftarrow A(\vec{Y})}$. Recall that $A(\vec{Y})$ is the head of $r$ and that $r$ is the rule associated with $v$. 
%Let $\phi$ be the composition of the MGUs that are computed at each step of Definition~\ref{definition:EP-rewriting}. 
%For an answer $\sigma$ to ${\rew(Q,G_{\preceq v})}$ over $B$, let $\sigma^{\phi}$ be the answer be the extension of $\sigma$ that additionally comprises the mappings ${X \mapsto \sigma(\phi(X))}$, 
%for each variable $X$ of $Q$ not occurring in ${\rew(Q,G_{\preceq v})}$.
%We show the correspondence between the facts associated with $v$ and the answers to ${\rew(Q,G_{\preceq v})}$ on $B$.
%
%\begin{lemma}\label{lemma:EP-rewriting}   
%	$v(B)$ comprises exactly a fact ${\sigma^{\phi}(Q)}$, 
%	for each answer $\sigma$ to ${\rew(Q,G_{\preceq v})}$ over $B$. 
%\end{lemma}
%
%We refer to ${\rew(Q,G_{\preceq v})}$ as the TG-rewriting of $v$. 
%
%Using Lemma~\ref{lemma:EP-rewriting}, we can reduce the problem of identifying nodes that can discarded from the TG to the problem of query containment.
%The above implies a simple technique for minimizing TGs of Datalog programs. 
 
%Let $\lambda$ be a mapping from the free variables $\vec{x}_1$ (ordered according to some canonical ordering) 
%of $Q_1$ into distinct fresh constants and 
%$I$ be the instance comprising exactly a fact $\lambda(\alpha)$ for each atom $\alpha$ in $Q_1$.  
%
%\begin{theorem}
%	(From \cite{Cali:2013:TIC:2591248.2591252}) $Q_1$ is contained in $Q_2$ iff ${\lambda(\vec{x}_1) \in Q_2(I)}$. 
%\end{theorem}
 
\begin{definition}\label{definition:minimizationDatalog}
	The EG $\mathsf{minDatalog}(G)$ is obtained from a TG $G$ of a program $P$ by exhaustively applying the steps below. 
	For each pair of nodes ${v,v'}$, where (i) $v$ is of the same of higher depth than $v'$, 
	(ii) $v$ defines the same predicate with $v'$ and (iii) the TG rewriting of $v$
	 is contained in the TG rewriting of $\head{v'}$, then: 
	(i) remove the node $v$ from $\nodes{G}$; and add an edge ${v' \rightarrow_j u}$, for each edge ${v \rightarrow_j u}$ occurring in $G$.
\end{definition}

The above procedure is sound. Furthermore, the computed TG is minimal in terms of the number of nodes. 

\begin{restatable}{theorem}{thmminimizeDatalog}\label{theorem:minimizeDatalog}
	For each TG $G$ of a program $P$, the graph $\mathsf{minDatalog}(G)$ is a TG for $P$. 
	Furthermore, each other TG for $P$ has at least as many nodes as $\mathsf{minDatalog}(G)$.  
\end{restatable}

We demonstrate an example of the minimization algorithm in the appendix.

Notice that our rewriting algorithm is different from previous work query rewriting, e.g., \cite{DBLP:journals/tods/GottlobOP14}. However, there the objective is to compute 
the perfect rewriting of a first-order rewritable CQ, while we aim at computing the CQ whose answers relate to the data stored in a specific node. 
  

==> sections/table-chasebench-rdfs.tex <==
%\begin{table*}[tb]
%    \centering
%    \scriptsize
%    \begin{adjustbox}{max width=\textwidth}
%    {\color{blue}
%        \input sections/table-chasebench.tex
%    }
%    \end{adjustbox}
%    \caption{{\color{blue}\chaseBench scenarios. Time is in s and memory in MB.}}
%    %\vspace{-1em}
%    \label{tab:chaseBench}
%
%    \centering
%    \scriptsize
%    \begin{adjustbox}{max width=\textwidth}
%    {\color{blue}
%        \input sections/table-rdfs.tex
%     }
%    \end{adjustbox}
%    \caption{{\color{blue}RDFS scenarios. Time is in sec and memory in MB.}}
%    \label{tab:rdfs}
%\end{table*}


==> sections/table-datalog-chasebench-triggers.tex <==
\begin{table}[tb]
    \centering
    \scriptsize
    \begin{adjustbox}{max width=\columnwidth}
    {\color{blue}}
    \input sections/table-triggers.tex
    \end{adjustbox}
    \vspace{0.2cm}
    \caption{{\#Triggers in millions for VLog and GLog on the Datalog and \chaseBench scenarios.}}
    \label{tab:triggers}
%\vspace{-1em}
\end{table}

